Multi-physics modeling of non-equilibrium phenomena in inductively coupled plasma discharges: Part I. A state-to-state approach

This work presents a vibrational and electronic state-to-state model for nitrogen plasma implemented within a multi-physics modular computational framework to study non-equilibrium effects in inductively coupled plasma (ICP) discharges. Within the computational framework, the set of vibronic (i.e., vibrational and electronic) master equations are solved in a tightly coupled fashion with the flow governing equations. This tight coupling eliminates the need for invoking any simplifying assumptions when computing the state of the plasma, thereby ensuring a higher degree of physical fidelity. To mitigate computational complexity, a maximum entropy coarse-graining strategy is deployed, effectively truncating the internal state space. The efficacy of this reduced StS model is empirically substantiated through zero-dimensional isochoric simulations. In these simulations, the results obtained from the reduced-order model are rigorously compared against those obtained from the full StS model, thereby confirming the accuracy of the reduced StS framework. The developed Coarse-grained StS model was employed to study the plasma discharge within the VKI Plasmatron facility. Our results reveal pronounced discrepancies between the plasma flow fields obtained from StS simulations and those derived from Local Thermodynamic Equilibrium (LTE) models, which are conventionally used in the simulation of such facilities. The analysis demonstrates a substantial departure of the internal state populations of atoms and molecules from the Boltzmann distribution. These nonequilibrium effects have important consequences on the energy coupling dynamics, thereby impacting the overall morphology of the plasma discharge. A deeper analysis of the results demonstrates that the population distribution is in a Quasi-Steady-State in the hot plasma core.

==> compilePDF <==
#!/bin/bash

NAME="main"
TEX_FILE=$NAME.tex
PDF_FILE=$NAME.pdf
LOG_FILE=$NAME.log
AUX_FILE=$NAME.aux
BBL_FILE=$NAME.bbl

rm -f $LOG_FILE $AUX_FILE 

# Convert EPS files to PDF
#find Figures -name "*.eps" -exec epstopdf {} \;

# Compile LaTeX document
#pdflatex $TEX_FILE
#bibtex $NAME
#pdflatex $TEX_FILE
#pdflatex $TEX_FILE

# Compile LaTeX document with LuaLaTeX and --shell-escape flag
pdflatex --shell-escape $TEX_FILE
bibtex $NAME
pdflatex --shell-escape $TEX_FILE
pdflatex --shell-escape $TEX_FILE

rm -f $LOG_FILE $AUX_FILE


